Algebraic perspectives on signomial optimization

Signomials are obtained by generalizing polynomials to allow for arbitrary real exponents. This generalization offers great expressive power, but has historically sacrificed the organizing principle of ``degree'' that is central to polynomial optimization theory. We reclaim that principle here through the concept of signomial rings, which we use to derive complete convex relaxation hierarchies of upper and lower bounds for signomial optimization via sums of arithmetic-geometric exponentials (SAGE) nonnegativity certificates. The Positivstellensatz underlying the lower bounds relies on the concept of conditional SAGE and removes regularity conditions required by earlier works, such as convexity and Archimedeanity of the feasible set. Through worked examples we illustrate the practicality of this hierarchy in areas such as chemical reaction network theory and chemical engineering. These examples include comparisons to direct global solvers (e.g., BARON and ANTIGONE) and the Lasserre hierarchy (where appropriate). The completeness of our hierarchy of upper bounds follows from a generic construction whereby a Positivstellensatz for signomial nonnegativity over a compact set provides for arbitrarily strong outer approximations of the corresponding cone of nonnegative signomials. While working toward that result, we prove basic facts on the existence and uniqueness of solutions to signomial moment problems.

==> problems/Fl1999_ex721.tex <==
\iffalse
    This appears as Problem 7.2.1 in Floudas et al, 1999.
    Floudas et al cite Dembo, 1976.
    
    This appears in Dembo, 1976 as Problem 3.
    Dembo states that the problem is taken from Bracken and McCormick ("Selected applications of nonlinear programming", 1968, pp. 37 -- 45) after eliminating equality constraints through substitution of variables.

    Bracken and McCormick dedicate Chapter 4 of their book to this problem. They state that the problem
    was described by Sauer, Colville, and Burwick [3]. That reference is not available online. Google Scholar
    can produce the citation:
    
        @article{sauer1964computer,
      title={Computer points way to more profits},
      author={Sauer, RN and Colville, AR and Burwick, CW},
      journal={Hydrocarbon Processing},
      volume={84},
      number={2},
      year={1964}
    }
\fi

%\begin{align}
%\min_{\vct{t} \in \R^7_{++}} 
 %           &~    c_1 t_1 + c_2 t_1 t_6 + c_3 t_3 + c_4 t_2 + c_5 - c_6 t_3 t_5                    \\
%&~ 1 \geq c_{7} t_{6}^{2}+c_{8} t_{1}^{-1} t_{3}-c_{9} t_{6} \nonumber \\
%&~ 1 \geq c_{10} t_{1} t_{3}^{-1}+c_{11} t_{1} t_{3}^{-1} t_{6}-c_{12} t_{1} t_{3}^{-1} t_{6}^{2} \nonumber \\
%&~ 1 \geq c_{13} t_{6}^{2}+c_{14} t_{5}-c_{15} t_{4}-c_{16} t_{6} \nonumber \\
%&~ 1 \geq c_{17} t_{5}^{-1}+c_{18} t_{5}^{-1} t_{6}+c_{19} t_{4} t_{5}^{-1}-c_{20} t_{5}^{-1} t_{6}^{2} \nonumber \\
%&~ 1 \geq c_{21} t_{7}+c_{22} t_{2} t_{3}^{-1} t_{4}^{-1}-c_{23} t_{2} t_{3}^{-1} \nonumber \\
%&~ 1 \geq c_{24} t_{7}^{-1}+c_{25} t_{2} t_{3}^{-1} t_{7}^{-1}-c_{26} t_{2} t_{3}^{-1} t_{4}^{-1} t_{7}^{-1} \nonumber \\
%&~ 1 \geq c_{27} t_{5}^{-1}+c_{28} t_{5}^{-1} t_{7} \nonumber \\
%&~ 1 \geq c_{29} t_{5}-c_{30} t_{7} \nonumber \\
%&~ 1 \geq c_{31} t_{3}-c_{32} t_{1} \nonumber \\
%&~ 1 \geq c_{33} t_{1} t_{3}^{-1}+c_{34} t_{3}^{-1} \nonumber \\
%&~ 1 \geq c_{35} t_{2} t_{3}^{-1} t_{4}^{-1}-c_{36} t_{2} t_{3}^{-1} \nonumber \\
%&~ 1 \geq c_{37} t_{4}+c_{38} t_{2}^{-1} t_{3} t_{4} \nonumber \\
%&~ 1 \geq c_{39} t_{1} t_{6}+c_{40} t_{1}-c_{41} t_{3} \nonumber \\
%&~ 1 \geq c_{42} t_{1}^{-1} t_{3}+c_{43} t_{1}^{-1}-c_{44} t_{6} \nonumber \\
%&~ (2000, 120, 3500, 93, 95, 12, 162) \geq \vct{t} \geq 1500, 1, 3000, 85, 90, 3, 145)  \nonumber
%\end{align}

%\begin{align}
%\min_{\vct{t} \in \R^7_{++}} 
%            &~    c_1 t_1 + c_2 t_1 t_6 + c_3 t_3 + c_4 t_2 + c_5 - c_6 t_3 t_5                    \\
%&~ 1 - c_{7} t_{6}^{2}- c_{8} t_{1}^{-1} t_{3} + c_{9} t_{6} \geq 0 \nonumber \\
%&~ 1 - c_{10} t_{1} t_{3}^{-1}- c_{11} t_{1} t_{3}^{-1} t_{6} + c_{12} t_{1} t_{3}^{-1} t_{6}^{2} \geq 0 \nonumber \\
%&~ 1 - c_{13} t_{6}^{2}- c_{14} t_{5} + c_{15} t_{4} + c_{16} t_{6} \geq 0 \nonumber \\
%&~ 1 - c_{17} t_{5}^{-1}- c_{18} t_{5}^{-1} t_{6}- c_{19} t_{4} t_{5}^{-1} + c_{20} t_{5}^{-1} t_{6}^{2} \geq 0 \nonumber \\
%&~ 1 - c_{21} t_{7}- c_{22} t_{2} t_{3}^{-1} t_{4}^{-1} + c_{23} t_{2} t_{3}^{-1} \geq 0 \nonumber \\
%&~ 1 - c_{24} t_{7}^{-1}- c_{25} t_{2} t_{3}^{-1} t_{7}^{-1} + c_{26} t_{2} t_{3}^{-1} t_{4}^{-1} t_{7}^{-1} \geq 0 \nonumber \\
%&~ 1 - c_{27} t_{5}^{-1}- c_{28} t_{5}^{-1} t_{7} \geq 0 \nonumber \\
%&~ 1 - c_{29} t_{5} + c_{30} t_{7} \geq 0 \nonumber \\
%&~ 1 - c_{31} t_{3} + c_{32} t_{1} \geq 0 \nonumber \\
%&~ 1 - c_{33} t_{1} t_{3}^{-1}- c_{34} t_{3}^{-1} \geq 0 \nonumber \\
%&~ 1 - c_{35} t_{2} t_{3}^{-1} t_{4}^{-1} + c_{36} t_{2} t_{3}^{-1} \geq 0 \nonumber \\
%&~ 1 - c_{37} t_{4}- c_{38} t_{2}^{-1} t_{3} t_{4} \geq 0 \nonumber \\
%&~ 1 - c_{39} t_{1} t_{6}- c_{40} t_{1} + c_{41} t_{3} \geq 0 \nonumber \\
%&~ 1 - c_{42} t_{1}^{-1} t_{3}- c_{43} t_{1}^{-1} + c_{44} t_{6} \geq 0 \nonumber \\
%&~ (2000, 120, 3500, 93, 95, 12, 162) \geq \vct{t} \geq (1500, 1, 3000, 85, 90, 3, 145)  \nonumber
%\end{align}

%\begin{align}
%\min_{\vct{t} \in \R^7_{++}} 
%            &~    c_1 t_1 + c_2 t_1 t_6 + c_3 t_3 + c_4 t_2 + c_5 - c_6 t_3 t_5                    \\
%&~ 1 - c_{7} t_{6}^{2}- c_{8} t_{1}^{-1} t_{3} + c_{9} t_{6} \geq 0 \nonumber \\
%&~ \textcolor{blue}{ t_1 - c_{7} t_1 t_{6}^{2}- c_{8} t_{3} + c_{9} t_1 t_{6} \geq 0 } \nonumber \\
%&~ 1 - c_{10} t_{1} t_{3}^{-1}- c_{11} t_{1} t_{3}^{-1} t_{6} + c_{12} t_{1} t_{3}^{-1} t_{6}^{2} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_3 - c_{10} t_{1} - c_{11} t_{1} t_{6} + c_{12} t_{1} t_{6}^{2} \geq 0} \nonumber \\
%&~ 1 - c_{13} t_{6}^{2}- c_{14} t_{5} + c_{15} t_{4} + c_{16} t_{6} \geq 0 \nonumber \\
%&~ \textcolor{blue}{1 - c_{13} t_{6}^{2}- c_{14} t_{5} + c_{15} t_{4} + c_{16} t_{6} \geq 0} \nonumber \\
%&~ 1 - c_{17} t_{5}^{-1}- c_{18} t_{5}^{-1} t_{6}- c_{19} t_{4} t_{5}^{-1} + c_{20} t_{5}^{-1} t_{6}^{2} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_5 - c_{17} - c_{18} t_{6}- c_{19} t_{4} + c_{20} t_{6}^{2} \geq 0} \nonumber \\
%&~ 1 - c_{21} t_{7}- c_{22} t_{2} t_{3}^{-1} t_{4}^{-1} + c_{23} t_{2} t_{3}^{-1} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_3 t_4 - c_{21} t_3 t_4 t_7 - c_{22} t_{2} + c_{23} t_{2} t_4 \geq 0} \nonumber \\
%&~ 1 - c_{24} t_{7}^{-1}- c_{25} t_{2} t_{3}^{-1} t_{7}^{-1} + c_{26} t_{2} t_{3}^{-1} t_{4}^{-1} t_{7}^{-1} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_3 t_4 t_7 - c_{24} t_3 t_4 - c_{25} t_{2} t_{4} + c_{26} t_{2} \geq 0} \nonumber \\
%&~ 1 - c_{27} t_{5}^{-1}- c_{28} t_{5}^{-1} t_{7} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_5 - c_{27} - c_{28} t_{7} \geq 0} \nonumber \\
%&~ 1 - c_{29} t_{5} + c_{30} t_{7} \geq 0 \nonumber \\
%&~ \textcolor{blue}{1 - c_{29} t_{5} + c_{30} t_{7} \geq 0} \nonumber \\
%&~ 1 - c_{31} t_{3} + c_{32} t_{1} \geq 0 \nonumber \\
%&~ \textcolor{blue}{1 - c_{31} t_{3} + c_{32} t_{1} \geq 0} \nonumber \\
%&~ 1 - c_{33} t_{1} t_{3}^{-1}- c_{34} t_{3}^{-1} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_3 - c_{33} t_{1} - c_{34} \geq 0} \nonumber \\
%&~ 1 - c_{35} t_{2} t_{3}^{-1} t_{4}^{-1} + c_{36} t_{2} t_{3}^{-1} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_3 t_4 - c_{35} t_{2} + c_{36} t_{2} t_4 \geq 0} \nonumber \\
%&~ 1 - c_{37} t_{4}- c_{38} t_{2}^{-1} t_{3} t_{4} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_2 - c_{37} t_2 t_{4} - c_{38} t_{3} t_{4} \geq 0} \nonumber \\
%&~ 1 - c_{39} t_{1} t_{6}- c_{40} t_{1} + c_{41} t_{3} \geq 0 \nonumber \\
%&~ \textcolor{blue}{1 - c_{39} t_{1} t_{6}- c_{40} t_{1} + c_{41} t_{3} \geq 0} \nonumber \\
%&~ 1 - c_{42} t_{1}^{-1} t_{3}- c_{43} t_{1}^{-1} + c_{44} t_{6} \geq 0 \nonumber \\
%&~ \textcolor{blue}{t_1 - c_{42} t_{3}- c_{43} + c_{44} t_1 t_{6} \geq 0} \nonumber \\
%&~ (2000,\, 120,\, 3500,\, 93,\, 95,\, 12,\, 162) - \vct{t} \geq \vct{0} \nonumber \\
%&~ \vct{t} - (1500,\, 1,\, 3000,\, 85,\, 90,\, 3,\, 145) \geq \vct{0}. \nonumber
%\end{align}

\subsection{A benchmark in alkylation process design}

Our next problem captures the design of an alkylation process in chemical engineering.
A detailed derivation of the original model (in ten variables) may be found in \cite{bracken1968selected} and the now-standard formulation (in seven variables) can be found in \cite[7.2.1]{Floudas1999}.
In order to make comparisons between SAGE relaxations and Moment-SOS relaxations we have cleared denominators in the signomial program \cite[7.2.1]{Floudas1999} to obtain a cubic polynomial optimization problem.
All coefficients in the formulation are positive and are given in the appendix.

\begin{align}
\min_{\vct{t} \in \R^7_{++}} 
            &~    c_1 t_1 + c_2 t_1 t_6 + c_3 t_3 + c_4 t_2 + c_5 - c_6 t_3 t_5                   \label{prob:ex2} \\
\text{s.t.} &~ t_1 - c_{7} t_1 t_{6}^{2}- c_{8} t_{3} + c_{9} t_1 t_{6} \geq 0 \nonumber \\
&~ t_3 - c_{10} t_{1} - c_{11} t_{1} t_{6} + c_{12} t_{1} t_{6}^{2} \geq 0 \nonumber \\
&~ 1 - c_{13} t_{6}^{2}- c_{14} t_{5} + c_{15} t_{4} + c_{16} t_{6} \geq 0 \nonumber \\
&~ t_5 - c_{17} - c_{18} t_{6}- c_{19} t_{4} + c_{20} t_{6}^{2} \geq 0 \nonumber \\
&~ t_3 t_4 - c_{21} t_3 t_4 t_7 - c_{22} t_{2} + c_{23} t_{2} t_4 \geq 0 \nonumber \\
&~ t_3 t_4 t_7 - c_{24} t_3 t_4 - c_{25} t_{2} t_{4} + c_{26} t_{2} \geq 0 \nonumber \\
&~ t_5 - c_{27} - c_{28} t_{7} \geq 0 \qquad 1 - c_{29} t_{5} + c_{30} t_{7} \geq 0 \nonumber \\
&~ 1 - c_{31} t_{3} + c_{32} t_{1} \geq 0 \qquad t_3 - c_{33} t_{1} - c_{34} \geq 0 \nonumber \\
&~ t_3 t_4 - c_{35} t_{2} + c_{36} t_{2} t_4 \geq 0 \qquad t_2 - c_{37} t_2 t_{4} - c_{38} t_{3} t_{4} \geq 0 \nonumber \\
&~ 1 - c_{39} t_{1} t_{6}- c_{40} t_{1} + c_{41} t_{3} \geq 0 \nonumber \\
&~ t_1 - c_{42} t_{3}- c_{43} + c_{44} t_1 t_{6} \geq 0 \nonumber \\
&~ (2000,\, 120,\, 3500,\, 93,\, 95,\, 12,\, 162) - \vct{t} \geq \vct{0} \nonumber \\
&~ \vct{t} - (1500,\, 1,\, 3000,\, 85,\, 90,\, 3,\, 145) \geq \vct{0}. \nonumber
\end{align}



In order to reflect the polynomial structure in \eqref{prob:ex2} we set $\cA = \{\vct{0},\vct{\delta}_1,\ldots,\vct{\delta}_7\}$.
We approach this problem first through conditional SAGE.
Let $X$ be the set defined by the seventeen signomial inequalities $g(\vct{x}) \geq 0$ where $g$ has exactly one positive term, and have $G$ include all twenty-eight constraints.
Table \ref{tab:ex2:original} shows the results of using MOSEK 9.2 to compute $f_K^{(3)}$ and $f_K^{(4)}$ for \eqref{prob:ex2}.
The reported solutions are feasible up to relative error at most $10^{-8}$, however the primal solutions exhibit substantial absolute constraint violation.


\begin{table}[ht!]
    \caption{MOSEK solution summary for SAGE relaxations to Problem \eqref{prob:ex2}. The primal and dual objectives agree to six significant digits. The four-tuples give a solution's $\ell_{\infty}$-norm, then violations of elementwise affine constraints, violations of bound constraints, and violations of conic constraints.}
    \centering
    \begin{tabular}{ccccc} % use \textcolor{white}{1} to get proper spacing.
    $d$ & objective & time & primal soln. norm \& viols. & dual soln. norm \& viols.  \\ \hline
      3 & 1224.52 & \textcolor{white}{00}8.64 & $(1\cdot 10^{8},\, 3\cdot 10^{-2},\, 3\cdot 10^{-3},\, 0)$ & $(3\cdot 10^{10},\, 0,\, 8\cdot 10^{-6},\, 0)$  \\
      4 & 1285.98 & 104.45 & $(8\cdot 10^{7},\, 2\cdot 10^{-1},\, 1\cdot 10^{-1},\, 0)$ & $(1\cdot 10^{10},\, 0,\, 2\cdot 10^{-6},\, 0)$ \\
    \end{tabular}
    \label{tab:ex2:original}
\end{table}

The solution quality data in Table \ref{tab:ex2:original} lead us to speculate that (1) the reported objective is larger than actually possible for a feasible primal solution and (2) the given dual solution is actually suboptimal.
We can validate this speculation by considering a rescaled version of the problem.
Specifically, we consider the change of variables
\[
    %\vct{t} \leftarrow 10\left(\frac{t_1}{2000},\, \frac{t_2}{120},\, \frac{t_3}{3500},\, \frac{t_4}{93},\, \frac{t_5}{95},\, \frac{t_6}{12},\, \frac{t_7}{162}\right)
    \vct{\hat{t}} \leftarrow (t_i u_i\,/\,10)_{i=1}^7 \quad \text{ for } \quad \vct{u} = (2000,\, 120,\, 3500,\, 93,\, 95,\, 12,\, 162)
\]
When considered in terms of exponential-form signomials this amounts to an affine shift $\vct{\hat{x}} \leftarrow \vct{x} - \log(10/\vct{u})$.
Table \ref{tab:ex2:rescaled} provides bounds and solver runtimes for this rescaled problem using both $X$-SAGE (conditional SAGE) and $\R^n$-SAGE (ordinary SAGE).
Applying solution recovery to the dual $X$-SAGE relaxation with $d=4$ produces a de-scaled solution
\[
    \vct{t}^\star \approx (1698.192,~  53.662,~ 3031.305,~   90.109,~   95.000,~   10.500,~  153.540)
    %\begin{cases}
        %array([1698.19,   53.66, 3031.31,   90.11,   95.  ,   10.5 ,  153.54])
    %    array([1698.19,   53.66, 3031.31,   90.11,   95.  ,   10.5 ,  153.54])
    %\end{cases}
\]
that is feasible within absolute error $3 \cdot 10^{-7}$ and satisfies $f(\log \vct{t}^\star) \approx 1227.23$.
The matching $X$-SAGE and $\R^n$-SAGE bounds show this is essentially optimal.
Note that in contrast to the runtime performance of $X$-SAGE and $\R^n$-SAGE relaxations for Problem \eqref{prob:ex1}, here the $X$-SAGE approach solves Problem \eqref{prob:ex2} over eight times faster than the $\R^n$-SAGE approach.

\begin{table}[ht!]
    \caption{SAGE bounds and solve times for the rescaled version of Problem \eqref{prob:ex2}.}
    \centering
    \begin{tabular}{c|cc|cc|} % use \textcolor{white}{2} to get proper spacing.
     & \multicolumn{2}{c}{$\cA$-degree $d$ SAGE bound} & \multicolumn{2}{|c|}{solver runtime} \\ 
    $d$ & conditional & ordinary & conditional & ordinary  \\ \hline
      3 & 1206.86 & 1125.12 & \textcolor{white}{2}3.83 & \textcolor{white}{22}2.83  \\
      4 & 1227.23 & 1224.98 & 50.56 & \textcolor{white}{2}84.12  \\
      %      4 & 1227.2265 & 1224.9820 & 50.5623 & \textcolor{white}{2}84.1217  \\
      5 & - & 1227.23 & - & 429.43 \\
      % 5 & - & 1227.2259 & - & 429.4254 \\
    \end{tabular}
    \label{tab:ex2:rescaled}
\end{table}

==> problems/rm1978_p19.tex <==
%\begin{align*}
%    f(\vct{t}) &= 2.0425\, t_{1}^{0.782} + 52.25\, t_{2} + 192.85\, t_{2}^{0.9} + 5.25\, t_{2}^3 + 61.465\, t_{6}^{0.467} \\
%    & \qquad + 0.01748\,  t_{3}^{1.33} / t_{4}^{0.8} + 100.7\, t_{4}^{0.546} + 3.66 {\cdot 10}^{-10} \, t_{3}^{2.85}/ t_{4}^{1.7} \\
%    & \qquad + 0.00945\, t_{5} + 1.06 {\cdot 10}^{-10}\, t_{5}^{2.8}/t_{4}^{1.8} + 116\, t_{6} - 205\, t_{6} t_{7} - 278\, t_{2}^3 t_{7} 
%\end{align*}

\begin{align*}
    \min_{\vct{t} \in \R^8_{++}} ~~& 2.0425\, t_{1}^{0.782} + 52.25\, t_{2} + 192.85\, t_{2}^{0.9} + 5.25\, t_{2}^3 + 61.465\, t_{6}^{0.467} \\[-0.75em]
    & \qquad + 0.01748\,  t_{3}^{1.33} / t_{4}^{0.8} + 100.7\, t_{4}^{0.546} + 3.66 {\cdot 10}^{-10} \, t_{3}^{2.85}/ t_{4}^{1.7} \\
    & \qquad + 0.00945\, t_{5} + 1.06 {\cdot 10}^{-10}\, t_{5}^{2.8}/t_{4}^{1.8} + 116\, t_{6} - 205\, t_{6} t_{7} - 278\, t_{2}^3 t_{7} \\[0.25em]
    \text{s.t.}~~ & 1 - 129.4/t_{2}^3 - 105/t_{6} \geq 0 \\
    & 1 - 1.03\cdot 10^5 \, t_{2}^3 t_{7}/(t_{3} t_{8}) - 1.2\cdot 10^6 /(t_{3} t_{8}) \geq 0 \\
    & 1 - 4.68\, t_{2}^3/t_{1} - 61.3\, t_{2}^2/t_{1} - 160.5\, t_{2}/t_{1} \geq 0 \\
    & 1 - 1.79\, t_{7} - 3.02\, t_{2}^3 t_{7}/t_{6} - 35.7\, /t_{6} - 1 \geq 0 \\
    & 1000 - 1.22\, t_{3} t_{8}/(t_{4}^{0.2} t_{5}^{0.8}) - 1.67\, t_{8} t_{3}^{0.4}/ t_{4}^{0.43} - 3.6 {\cdot 10}^{-2}\, t_{3} t_{8}/t_{4} - 2\, t_{3} t_{8}/t_{5} - 4\, t_{8} \geq 0
\end{align*}


==> problems/rm1978p9_geo.tex <==
% gts_1__lo.. 0 =l= 0.05*t_1_ + 1 + t_2_ ** 0.05*(-0.76729999999999998) ;
% f.. GAMS_OBJECTIVE =e= t_1_ ** 0.84999999999999998*3.7 + 1.985*t_1_ + t_2_ ** (-0.75)*700.2999999999999 ;

\begin{align*}
    \min_{\vct{t} \in \R^2_{++}} 
            &~    3.7 t_1^{0.85} + 1.985 t_1 + 700.3 t_2^{-0.75}                    \\
        \text{s.t. }    &~ 1 + 0.05 t_1 -0.7673 t_2^{0.05} \geq 0
\end{align*}


\iffalse

Note that both $f$ and $g$ are increasing in $x_1$ and decreasing in $x_2$.
Based on this we can infer that any local minimizer $\vct{x}^\star$ satisfies $x_2^\star = 20\log\left(( 0.05\exp(x_1^\star) + 1)/0.7673\right)$.
The expression for $x_2$ as a function of $x_1$ can be substituted into $f(x_1,x_2)$.
After performing this substitution, we solve the resulting unconstrained univariate minimization problem to find $(f,\{g\})_{\R^2}^\star \approx 11.9643$.

\vspace{1cm}

We consider these signomials in the ring induced by
\[
    \cA = \begin{bmatrix}
             0   &   0 &   0  &  0.85 &  1  \\
            -0.75  &  0  &  0.05 &  0   &  0  
            \end{bmatrix}^\top \in \R^{5 \times 2}
\]
so that $\deg_{\cA}(f) = \deg_{\cA}(g) = 1$.

Despite this problem's simplicity and our ability to solve it nearly by hand, it is known to create difficulties for numerical algorithms.
Claimed optimal objective values include
\begin{itemize}
    \item \cite{RM1978}-9. Solution evaluates to 11.96392; violates constraints by 5e-6. Other notes: (1) used \textbf{local} optimization algorithms, (2) sourced from the 1970 PhD thesis of Rijckaert, (3) reported objective value was 11.91.
    \item \cite{WL2005}-4. Claimed objective: 11.9538. Other notes (1) added bound constraints and epigraph variable, (2) sourced from a 1990 publication.
    \item \cite{Shen2008}-3.
    Claimed objective: 12.0475.
    Other notes: (1) same formulation as \cite{WL2005}, (2) solution evaluates to 11.96477 and is strictly feasible.
    \item \cite{HSC2014}-2. Claimed objective: 7.8922. Other notes: same formulation as \cite{Shen2008}.
    \item \cite{MCW2019}. Claimed lower bound 11.7 (level (3,3,1) relaxation). Notes (1) claimed feasible solution value (11.9600) is an incorrect transcription of data from the experiments; the correct value should be 11.9643, (2) the bound 11.7 can be reproduced with a primal relaxation, but the dual relaxation gives something more like 11.03; the cause of this difference is not clear to me.
\end{itemize}

\vspace{1cm}

Flow: \cite{RM1978} found the global optimum with local solvers; don't certify as much. Then people looked at global optimization. As with us, proof of convergence with global optimization requires compactness. However, alternative methods are based on branch-and-bound, and hence often cannot meaningfully run without a compact feasible set (and known variable bounds). By adding explicit bounds, \cite{WL2005} report a solution with objective value 11.9538; this is infeasible by 1e-4. A feasibility-focused global optimization method found a solution with objective 12.0475 \cite{Shen2008}. Hu, Shen, and Chen report a solution with objective 7.822, but this violates the constraint by 0.036.
\fi
